Standard model anomalies: Lepton flavour non-universality, g-2 and W-mass

We critically analyze the body of results that hints to the existence of New Physics from possible violations of lepton universality observed by the LHCb experiment in the $\mu/e$ ratios $R_{K}$ and $R_{K^*}$ to the $g-2$ lepton anomalies. The analysis begins with a theoretical, in depth, study of the $\mu/e$ ratios $R_{K}$ and $R_{K^*}$ as well as the process $B_s \rightarrow \mu^+ \mu^-$. Here we consider the impact of complex Wilson coefficients and derive constraints on their imaginary and real parts. We then move to a comprehensive comparison with experimental results. We show that, by fitting a single Wilson coefficient, the deviations from the Standard Model are at the $4.7\sigma$ level when including only the hadronic insensitive observables while it increases to $6.1\sigma$ when including also the hadronic sensitive ones. When switching on all relevant Wilson coefficients and combining both hadronic sensitive and insensitive data into the fit, the deviation from the Standard Model peaks at $7.2\sigma$ and decreases at the $4.9\sigma$ level if we assume that the central values of $R_K$ and $R_{K^{\ast}}$ are taken to be unity. We further estimate other unaccounted for SM contributions and show that their inclusion still requires New Physics to fit the data. We then introduce the $g-2$ lepton anomalies as well as the most recent $W$-mass results. Different theoretical models are considered that can explain the discrepancies from the Standard Model. In the final part of our work we estimate the impact of the forthcoming data from LHCb (coming from LHC Run3) and Belle II, when it will have accumulated about $5~ab^{-1}$.

==> _Belle_II_predictions.tex <==
\begin{table*}[htb]
\begin{center}
 \caption{Expected errors on several selected observables in leptonic and semileptonic $B$ decays.} 
\label{tab:summ_wg1a}
\begin{tabularx}{\textwidth}{llXX}
\hline
Observables 						&  Belle   												&    \multicolumn{2}{c}{Belle II}  \\
                   						&  (2017) 												&    5 ab$^{-1}$ 	& 50 ab$^{-1}$ \\
\hline
$|V_{cb}|$ incl. 		    				& $42.2\cdot10^{-3} \cdot (1\pm 1.8\%)$ 							& $1.2\%$ 		& $-$ \\%1S
$|V_{cb}|$ excl. 					& $39.0\cdot10^{-3} \cdot (1\pm 3.0\%_{\rm ex.} \pm 1.4\%_{\rm th.})$  	& $1.8\%$ 		& $1.4\%$  \\%GGOU
$|V_{ub}|$ incl. 						& $4.47\cdot10^{-3} \cdot (1\pm 6.0\%_{\rm ex.} \pm 2.5\%_{\rm th.})$ 	& $3.4\%$ 		& $3.0\%$  \\
$|V_{ub}|$ excl. (WA)				& $3.65\cdot10^{-3} \cdot (1\pm 2.5\%_{\rm ex.} \pm 3.0\%_{\rm th.} )$ 	& $2.4\%$ 		& $1.2\%$ \\%fit
${\cal{B}}(B \to \tau\nu)$ [$10^{-6}$] 		& $91 \cdot (1 \pm 24\%)$						 				& $9\%$ 			& $4\%$ \\
${\cal{B}}(B \to \mu\nu)$ [$10^{-6}$] 		& $< 1.7$													& $20\%$ 			& $7$\%  \\
$R(B\to D\tau \nu)$ (Had. tag) 			& $0.374\cdot  (1\pm 16.5\%)$							 		& $6\%$ 			& $3\%$ \\
$R(B\to D^*\tau \nu)$ (Had. tag) 		& $0.296 \cdot (1\pm 7.4\%)$									& $3\%$ 			& $2\%$ \\
\hline
\end{tabularx}
\end{center}
\end{table*}


\begin{table*}[htp]
\caption{Belle II Golden/Silver observables for the pure-leptonic and the semi-leptonic $B$ decays. The theory column indicates the robustness against the theory uncertainties. The discovery column shows the integrated luminosity at which the discovery of new physics is possible. The Sys. limit column indicates at which integrated luminosity the experimental systematic uncertainty dominates. The vs LHCb/BESIII, Belle columns show the originality and the competitiveness against those experiments. The anomaly column indicates whether there is an existing hint of new physics and the NP columnshows whether the observable is sensitive to new physics models. }
\label{tab:summ_wg1b}
\begin{center}
\begin{tabularx}{\textwidth}{clcXXXXXX }
\hline
&\rot{30}{Process} & \rot{30}{Observable}   & \rot{30}{Theory} & \rot{30}{Sys. dom. (Discovery) [ab$^{-1}$]}  & \rot{30}{vs  LHCb }& \rot{30}{vs Belle} & \rot{30}{Anomaly} & \rot{30}{NP}   \\ 
\hline 
 \goldmedal & $B\to \pi \ell\nu_\ell$ 		& $|V_{ub}|$ 	& \threestar 	& \ 10-20 		& \threestar 	& \threestar 	& \twostar 	& \onestar \\ 
\goldmedal & $B\to X_u \ell\nu_\ell$		& $|V_{ub}|$ 	& \twostar 	& \ \ 2-10 		&\threestar 	& \twostar 	& \threestar 	& \onestar \\ 
\goldmedal & $B\to \tau \nu $ 			& $Br.$ 		& \threestar 	& $>$50~(2) 	&\threestar 	& \threestar 	& \onestar 	& \threestar \\ 
\goldmedal & $B\to \mu \nu $ 			& $Br.$ 		& \threestar 	& $>$50~(5) 	&\threestar 	& \threestar 	& \onestar 	& \threestar \\ 
\goldmedal & $B\to D^{(*)} \ell\nu_\ell $ 	& $|V_{cb}|$ 	& \threestar 	& \ \ 1-10 	&\threestar 	& \twostar 	& \twostar 	&\onestar \ \ \\ 
\goldmedal & $B\to X_c \ell\nu_\ell $ 		&  $|V_{cb}|$ 	& \threestar 	& \ \ 1-5 	&\threestar 	& \twostar 	& \twostar 	& \twostar \\ 
\goldmedal & $B\to D^{(*)} \tau\nu_\tau $ 	&  $R(D^{(*)})$	& \threestar 	& \ \ 5-10 	&\twostar 		& \threestar 	& \threestar 	& \threestar \\ 
\silvermedal & $B\to D^{(*)} \tau\nu_\tau $ &  $P_\tau$	& \threestar 	& \  15-20 	&\threestar 	& \threestar 	& \twostar 	& \threestar \\ 
\silvermedal & $B\to D^{**} \ell\nu_\ell $ 	&  $Br.$		& \onestar 	& \ \ - 	&\twostar 		& \threestar 	& \twostar 	& \ \ - \\ 
\hline
\end{tabularx}
\end{center}
\end{table*}%



\begin{table*}[htb]
\begin{center}
 \caption{Expected errors on several selected observables in radiative and electroweak penguin $B$ decays. Note that $50$ ab$^{-1}$ projections for $B_s$ decays are not provided as we do not expect to collect such a large $\Upsilon(5S)$ data set.} 
\label{tab:summ_wg2a}
\begin{tabularx}{\textwidth}{Xlll}
\hline
Observables 									&  Belle   												&    \multicolumn{2}{c}{Belle II}  \\
                   									&  (2017) 												&    5 ab$^{-1}$ 	& 50 ab$^{-1}$ \\
\hline
${\cal{B}}(B \to K^{*+}\nu \overline{\nu})$  				& $< 40 \times	 10^{-6}$									& 25\% 			& 9\% \\
${\cal{B}}(B\to K^{+}\nu \overline{\nu})$ 				& $< 19 \times	 10^{-6}$ 									& 30\% 			& 11\% \\
${A_{CP}}(B\to X_{s+d} \gamma)$~$[10^{-2}]$ 			& $2.2 \pm 4.0 \pm 0.8$								        & $1.5$ 			& $0.5$  \\
$S$($B \to K_S^0 \pi^0 \gamma$) 					& $-0.10 \pm 0.31 \pm 0.07$								& $0.11$ 			& $0.035$\\
$S$($B \to \rho \gamma$) 						& $-0.83 \pm 0.65 \pm 0.18$								& $0.23$ 			& $0.07$ \\
$A_{FB}(B\to X_s \ell^+ \ell^-)$ ($1<q^2<3.5$ GeV$^2/c^4$) & 26\% & 10\% & 3\%\\
%$C_7/C_9~(B\to X_s\ell\ell)$ 						& $\sim$20\%										        &  10\%   			&  5\%   \\
$Br(B\to K^+ \mu^+ \mu^-)/Br(B\to K^+ e^+ e^-)$ ($1<q^2<6$ GeV$^2/c^4$)			& 28\% & 11\% & 4\% \\ 
$Br(B\to K^{*+}(892) \mu^+ \mu^-)/Br(B\to K^{*+}(892) e^+ e^-)$ ($1<q^2<6$ GeV$^2/c^4$)			& 24\% & 9\% & 3\% \\ 
${\cal{B}}(B_s\to \gamma \gamma)$ 		& $<8.7\times 10^{-6}$												& 23\% 			& $-$\\
${\cal{B}}(B_s\to \tau \tau)$ [$10^{-3}$] 		        		& $-$ 							                                       	& $< 0.8$			& $-$ \\
\hline
\end{tabularx}
\end{center}
\end{table*}


\begin{table*}[htp]
%\renewcommand{\arraystretch}{1.2}
\caption{Belle II Golden/Silver observables for the radiative and the electroweak penguin $B$ decays. See the caption in Table \ref{tab:summ_wg1b} for more details. 
The precision limit of the $B\to X_s\gamma $ measurement estimated simply by estimating the point where the statistic uncertainties dominate. However, the systematic uncertainties may be further reduced by adding more data. 
}
\label{tab:summ_wg2b}
\begin{center}
\begin{tabularx}{\textwidth}{ c l c XXXXXX }
\hline
&\rot{30}{Process} & \rot{30}{Observable}   & \rot{30}{Theory} & \rot{30}{Sys. dom. (Discovery) [ab$^{-1}$]}  & \rot{30}{vs  LHCb }& \rot{30}{vs Belle} & \rot{30}{Anomaly} & \rot{30}{NP}   \\ 
\hline 
\goldmedal & $B\to K^{(*)}\nu\nu$ 		& $Br., F_L$ 				& \threestar 	& \ $>$50 	&\threestar 	& \threestar 	& \onestar 	& \twostar \\ 
\goldmedal & $B\to X_{s+d}\gamma $ 	& $A_{\rm CP}$ 		& \threestar 	& \ $>$50 	&\threestar 	& \threestar 	& \onestar		& \twostar \\ 
\goldmedal & $B\to X_d\gamma $ 		& $A_{\rm CP}$ 		& \twostar 	& \ $>$50 	& \threestar	& \threestar 	& \ \ - 		& \twostar \\ 
\goldmedal & $B\to K_S^0\pi^0\gamma $ 	& $S_{K_S^0\pi^0\gamma}$ & \twostar 	& \ $>$50 	&\twostar 		& \threestar 	& \onestar 	& \threestar \\ 
\goldmedal & $B\to \rho\gamma $ 		& $S_{\rho\gamma}$		& \twostar 	& \ $>$50 	&\threestar 		& \threestar 	& \ \ -		& \threestar\\ 
\goldmedal & $B\to X_s \ell^+\ell^-$	 		& $Br.$ 			& \threestar 	& \ $>$50 	& \threestar 	& \twostar 	& \twostar 	& \threestar \\ 
\goldmedal & $B\to X_s \ell^+\ell^-$	 		& $R_{X_s}$ 			& \threestar 	& \ $>$50 	& \threestar 	& \threestar 	& \twostar 	& \threestar \\ 
\goldmedal & $B\to K^{(*)}e^+e^- $                  	&  $R(K^{(*)})$                         	& \threestar    	& \ $>$50  &\twostar         	& \threestar    	& \threestar    	& \threestar \\
\silvermedal & $B\to X_s\gamma $ 		&  $Br.$				& \twostar 	& \ 1-5 	&\threestar 	& \onestar 	& \onestar 	& \twostar \\ 
\silvermedal & $B_{d, (s)}\to \gamma\gamma$ 	&  $Br., A_{\rm CP}$				& \twostar 	& \ $>$50 	&\twostar 		& \twostar 	& \ \ - 		& \twostar \\
\silvermedal & $B\to K^*e^+e^- $ 		&  $P_5^{\prime}$ 		& \twostar 	& \ $>$50 	&\threestar 		& \twostar 	& \threestar 	& \threestar \\ 
\silvermedal & $B\to K\tau \ell $ 			&  $Br.$				& \threestar 	& \  $>$50 &\twostar 		& \threestar 	& \twostar 	& \threestar \\ 
\hline
\end{tabularx}
\end{center}
\end{table*}%




\begin{table*}[htb]
\begin{center}

 \caption{Expected errors on several selected flavour observables 
with an integrated luminosity of 50~ab$^{-1}$ of Belle II 
data. Errors given in \%  represent relative errors. In the final column we denote where LHCb is expected to reach a highly competitive level of precision: if one experiment is expected to be slightly more accurate we list it first.} 
\small
\label{tab:summ}
\begin{tabularx}{0.9\linewidth}{lXXX}
\hline
Observables &  Expected the.~accuracy & Expected exp.~uncertainty & Facility (2025)   \\
\hline
UT angles \& sides\\
$\phi_1$ [$^\circ$]									& ***		& 0.4 	& Belle II \\ 
$\phi_2$ [$^\circ$] 									& **  		& 1.0 	& Belle II \\
$\phi_3$ [$^\circ$]									& *** 	& 1.0 	& LHCb/Belle II \\
%$S(B_s \to J/\psi \phi)$ 								& *** 	& 0.01 	& LHCb \\ 
%\hline
%UT sides \\
$|V_{cb}|$ incl. 		    								& *** 	& 1\% 	&Belle II\\
$|V_{cb}|$ excl. 									& *** 	& 1.5\% 	&Belle II \\
$|V_{ub}|$ incl. 										& **  		& 3\% 	&Belle II \\
$|V_{ub}|$ excl. 		  							& **  		& 2\% 	&Belle II/LHCb\\
\hline
$CP$ Violation\\
$S$($B \to \phi K^0$) 								& *** 	& 0.02 	&Belle II\\
$S$($B \to \eta' K^0$) 								& *** 	& 0.01 	&Belle II\\
%$S$($B \to K_S^0K_S^0K_S^0$) 			        			& 		& 		&Belle II\\
%$\beta_s^{\rm eff}$($B_s \to \phi \phi$)		[rad]			& ** 		& 0.1		&LHCb\\
%$\beta_s^{\rm eff}$($B_s \to K^{*0} \bar K^{*0}$)		[rad]	& ** 		& 0.1 	&LHCb\\
${\cal A}$($B \to K^0\pi^0$)[$10^{-2}$]					& *** 	& 4 		&Belle II\\
${\cal A}$($B \to K^+\pi^-$) [$10^{-2}$]					& *** 	& 0.20 	&LHCb/Belle II\\
%${\cal A}$($B \to \pi^+\pi^-$) 							& 		& 		&LHCb/Belle II\\
\hline
(Semi-)leptonic\\
${\cal{B}}(B \to \tau\nu)$ [$10^{-6}$] 						& ** 		& 3\%	&Belle II\\
${\cal{B}}(B \to \mu\nu)$ [$10^{-6}$] 						& ** 		& 7\%	&Belle II\\
$R(B\to D\tau \nu)$ 									& *** 	& 3\% 	&Belle II\\
$R(B\to D^*\tau \nu)$	  							& *** 	& 2\% 	&Belle II/LHCb\\
\hline
Radiative \& EW Penguins\\
${\cal{B}}(B\to X_s \gamma)$  							& ** 		& 4\% 	&Belle II\\
${A_{CP}}(B\to X_{s,d} \gamma)$~$[10^{-2}]$ 				& *** 	& 0.005 	& Belle II\\
$S$($B \to K_S^0 \pi^0 \gamma$) 						& *** 	& 0.03 	& Belle II\\
%$2\beta_s^{\rm eff}$($B_s \to \phi \gamma$) 				& *** 	& 0.05 	& LHCb\\
$S$($B \to \rho \gamma$) 							& **  		& 0.07 	& Belle II \\
${\cal{B}}(B_s\to \gamma \gamma)$ [$10^{-6}$] 			& ** 		& 0.3 	& Belle II \\
%\hline
%EW penguins\\
${\cal{B}}(B \to K^{*}\nu \overline{\nu})$ [$10^{-6}$] 			& *** 	& 15\% 	& Belle II \\
%${\cal{B}}(B\to K \nu \overline{\nu})$ [$10^{-6}$] 			& *** 	& 20\% 	& Belle II\\
%$C_7/C_9~(B\to X_s\ell\ell)$ 							& & & \\
$R(B\to K^*\ell\ell)$ 									& *** 	& 0.03 	& Belle II/LHCb\\
%${\cal{B}}(B_s\to \tau \tau)$ [$10^{-3}$] 					& *** 	& $<2$ 	& Belle II \\
%${\cal{B}}(B_s\to \mu \mu)$ 							& *** 	& 10\% 	& LHCb/Belle II\\
\hline
Charm \\
${\cal{B}}(D_s\to\mu\nu)$       							& *** 	& 0.9\%	& Belle II \\
${\cal{B}}(D_s\to\tau\nu)$    							& *** 	& 2\% 	& Belle II\\
%${\cal B}(D^0\to\gamma\gamma)~[10^{-6}]$   			&  \\
%Charm $CP$\\
%$A_{CP}(D^0\to K^+K^-)~[10^{-4}]$       					&  \\
%$\Delta A_{CP}(D^0\to K^+K^-)~[10^{-4}]$       			&  ** & 0.1 & LHCb\\
%$A_{\Gamma}~[10^{-2}]$       							&  \\
%$A_{CP}(D^0\to \pi^0\pi^0)$~[$10^{-2}$]        				&  \\
$A_{CP}(D^0\to K_S^0\pi^0)$~[$10^{-2}$]        				&  ** 		& 0.03 	& Belle II\\
%Charm Mixing\\
%$x(D^0\to K_S^0\pi^+\pi^-)$~[$10^{-2}$]        				&  \\
%$y(D^0\to K_S^0\pi^+\pi^-)$~[$10^{-2}$]        				&  \\
$|q/p|(D^0\to K_S^0\pi^+\pi^-)$               					&  *** 	& 0.03 	& Belle II \\
$A_{CP}(D^+\to \pi^+\pi^0)$~[$10^{-2}$]        				&  **		& 0.17	& Belle II \\
%$\phi(D^0\to K_S^0\pi^+\pi^-)$~[$^\circ$]     				&  *** 	& 4 		& Belle II \\
\hline
Tau\\
$\tau\to \mu\gamma$ [$10^{-10}$] 						& *** 	& $<50$ 	& Belle II\\
$\tau\to e\gamma$ [$10^{-10}$]   						& *** 	& $<100$ 	& Belle II\\
$\tau\to \mu\mu\mu$ [$10^{-10}$] 						& *** 	& $<3$ 	& Belle II/LHCb\\
\hline
\end{tabularx}
\end{center}
\end{table*}


\begin{table*}[htb]
\begin{center}
 \caption{Expected errors on several selected observables in radiative and electroweak penguin $B$ decays. Note that $50$ ab$^{-1}$ projections for $B_s$ decays are not provided as we do not expect to collect such a large $\Upsilon(5S)$ data set.} 
\label{tab:summ_wg2a}
\begin{tabularx}{\textwidth}{Xlll}
\hline
Observables 									&  Belle   												&    \multicolumn{2}{c}{Belle II}  \\
                   									&  (2017) 												&    5 ab$^{-1}$ 	& 50 ab$^{-1}$ \\
\hline
${\cal{B}}(B \to K^{*+}\nu \overline{\nu})$  				& $< 40 \times	 10^{-6}$									& 25\% 			& 9\% \\
${\cal{B}}(B\to K^{+}\nu \overline{\nu})$ 				& $< 19 \times	 10^{-6}$ 									& 30\% 			& 11\% \\
${A_{CP}}(B\to X_{s+d} \gamma)$~$[10^{-2}]$ 			& $2.2 \pm 4.0 \pm 0.8$								        & $1.5$ 			& $0.5$  \\
$S$($B \to K_S^0 \pi^0 \gamma$) 					& $-0.10 \pm 0.31 \pm 0.07$								& $0.11$ 			& $0.035$\\
$S$($B \to \rho \gamma$) 						& $-0.83 \pm 0.65 \pm 0.18$								& $0.23$ 			& $0.07$ \\
$A_{FB}(B\to X_s \ell^+ \ell^-)$ ($1<q^2<3.5$ GeV$^2/c^4$) & 26\% & 10\% & 3\%\\
%$C_7/C_9~(B\to X_s\ell\ell)$ 						& $\sim$20\%										        &  10\%   			&  5\%   \\
$Br(B\to K^+ \mu^+ \mu^-)/Br(B\to K^+ e^+ e^-)$ ($1<q^2<6$ GeV$^2/c^4$)			& 28\% & 11\% & 4\% \\ 
$Br(B\to K^{*+}(892) \mu^+ \mu^-)/Br(B\to K^{*+}(892) e^+ e^-)$ ($1<q^2<6$ GeV$^2/c^4$)			& 24\% & 9\% & 3\% \\ 
${\cal{B}}(B_s\to \gamma \gamma)$ 		& $<8.7\times 10^{-6}$												& 23\% 			& $-$\\
${\cal{B}}(B_s\to \tau \tau)$ [$10^{-3}$] 		        		& $-$ 							                                       	& $< 0.8$			& $-$ \\
\hline
\end{tabularx}
\end{center}
\end{table*}


\begin{landscape}
\begin{table*}[htb]
\begin{center}
 \caption{Projected precision of selected flavour physics measurements at Belle II and LHCb} 
\label{tab:2022}
\begin{tabularx}{1.25\textwidth}{p{0.25\textwidth}XXXXXXX}
\toprule
Observable	&  2022 & 2022 & Belle-II & Belle-II & LHCb & Belle-II & LHCb  \\
&  Belle (II),BaBar & LHcb & 5 ab$^{-1}$ & 50 ab$^{-1}$  & 23 ab$^{-1}$  & 250 ab$^{-1}$ & 300 ab$^{-1}$\\
\midrule
$\sin 2\beta /\phi_1$ & 0.03 & 0.04 & 0.012 & 0.005 & 0.011 & 0.002 & 0.003 \\
$\gamma/\phi_3$ & 13\textdegree & 5.4 \textdegree & 4.7 \textdegree & 1.5 \textdegree & 1.5 \textdegree & 0.4 \textdegree & 0.4 \textdegree \\
$\alpha/\phi_2$ & 4\textdegree & $-$ & 2 \textdegree & 0.6 \textdegree & $-$ & 0.3 \textdegree & $-$ \\
$|V_{ub}|/|V_{cb}|$ & 4.5\% & 6\% & 2\% & 1\% & 3\% & <1\% & 1\% \\
\midrule
$S_{CP}(B\rightarrow\eta ' K_S^0)$ & 0.08 & $-$ & 0.03 & 0.015 & $-$ & 0.007 & $-$\\
$A_{CP}(B\rightarrow\pi^0 K_S^0)$ & 0.15 & $-$ & 0.07 & 0.04 & $-$ & 0.02 & $-$\\
%$S_{CP}(B\rightarrow\eta '  K_S^0)$ & 0.15 & $-$ & 0.07 & 0.04 & $-$ & 0.02 & $-$\\
\midrule
$R(B\rightarrow K^*\ell^+\ell^- : 1<q^2<6 \,GeV^2)$  & 0.24 & 0.1 & 0.09 & 0.03 & 0.03 & 0.01 & 0.01 \\
$R(B\rightarrow D^*\tau\nu)$ & 6\% & 10\% & 3\% & 1.5\% & 3\% & <1\% & 1\% \\
$\mathcal{B}(B\rightarrow \tau\nu)$ & 24\% & $-$ & 9\% & 4\% & $-$ & <2\% & $-$ \\
$R(B\rightarrow K^*\nu\nu)$ & $-$ & $-$ & 25\% & 9\% & $-$ & 4\% & $-$ \\
\midrule
$\mathcal{B}(\tau\rightarrow e\gamma)UL$ & 120$\times 10^{-9}$& $-$ & 40$\times 10^{-9}$ & 12$\times 10^{-9}$& $-$ & 5$\times 10^{-9}$ & $-$ \\
$\mathcal{B}(\tau\rightarrow \mu\mu\mu)UL$ & 21$\times 10^{-9}$& 46$\times 10^{-9}$ & 3$\times 10^{-9}$ & 0.3$\times 10^{-9}$& 16$\times 10^{-9}$ & 0.06$\times 10^{-9}$ & 5$\times 10^{-9}$ \\
\bottomrule
\end{tabularx}
\end{center}
\end{table*}
\end{landscape}

